Non-average price impact in order-driven markets

We present a measurement of price impact in order-driven markets that does not require averages across executions or scenarios. Given the order book data associated with one single execution of a sell metaorder, we measure its contribution to price decrease during the trade. We do so by modelling the limit order book using state-dependent Hawkes processes, and by defining the price impact profile of the execution as a function of the compensator of a stochastic process in our model. We apply our measurement to a data set from NASDAQ, and we conclude that the clustering of sell child orders has a bigger impact on price than their sizes.

==> bm14_model.tex <==
\subsection{Model description}
Two aspects of the time evolution of the order-driven market are modelled:
trades and changes in the mid-price.
% As explained in Section \ref{sec.order-driven_markets}, 
Trades can in fact be identified with submissions of market orders, and we will do this here.

Four streams of arrival times are considered:
the stream $(\arrivalTimes[1]_j)_j$ of times when limit orders are executed on the bid side
(equivalently identified with the arrival times of sell market orders);
the stream  $(\arrivalTimes[2]_j)_j$ of times when limit orders are executed on the ask side
(equivalently identified with arrival times of buy market orders);
the stream  $(\arrivalTimes[3]_j)_j$ of times when the mid-price decreases;
the stream  $(\arrivalTimes[4]_j)_j$ of times when the mid-price increases. 
Correspondingly, these sequences of random times give rise to a four-dimensional counting process $\multiCountingProc=(\countingProc[1],\dots, \countingProc[4])$ with the following interpretation of its components:
\begin{itemize}
 \item $\countingProc[1](t)$ denotes the number of seller-initiated trades that happened before or at time $t$
(identified with the number of market orders arrived on the bid side of the order book by time $t$);
 \item $\countingProc[2](t)$ denotes the number of buyer-initiated trades that happened before or at time $t$
(identified with the number of market orders arrived on the ask side of the order book by time $t$);
 \item $\countingProc[3](t)$ denotes the number of downward jumps of the mid-price  that happened before or at time $t$;
 \item $\countingProc[4](t)$ denotes the number of upward jumps of the mid-price  that happened before or at time $t$.
\end{itemize}

Notice that $\countingProc[4]-\countingProc[3]$ is a proxy for the mid-price.
Indeed,
given the tick size $\tickSizeOfLOB$ of the limit order book and the initial position $\midprice_0$ of the mid-price,
 the paths $t\mapsto \midprice_0 +(\countingProc[4](t)-\countingProc[3](t))\tickSizeOfLOB$ and $t\mapsto \midprice_t$ will have discrepancies only when $\vert\delta\midprice(t)\vert \geq 2\tickSizeOfLOB$,
and this rarely happens (in particular for limit order books with large tick size).

The counting process $\multiCountingProc$ is assumed to be an ordinary Hawkes process,
hence it admits a continuous compensator with an intensity $\intensity[]=(\intensity[1],\dots,\intensity[4])$ of the type in equation \eqref{eq.intensity_ordHawkes}.
 We let $\baseRate$ be the $4$-dimensional vector of base rates, and we let $\hawkesKernel$ be the $4\times4$-dimensional matrix of Hawkes kernels.
 In the model of \cite{BM14haw}, the following assumptions are in place on the so-introduced four-dimensional Hawkes process:
\begin{assumption}\label{assumption.BM14}
 \begin{enumerate}[label={\emph{\roman{*}}.} , ref={\ref{assumption.BM14}.\emph{\roman{*}}}]
  \item\label{assumption.BM14.symmetric_baseRates} (symmetric base rates)
  $\baseRate_{2k-1}=\baseRate_{2k}$,  for $k=1,2$;
  \item\label{assumption.BM14.null_price-jumps_baseRates} (fully endogenous price jumps) $\baseRate_3 = \baseRate_4=0$;
  \item \label{assumption.BM14.symmetric_cross-excitation}(symmetric cross-excitation)
  $\hawkesKernel_{2k-1,2j}=\hawkesKernel_{2j,2k-1}$, for $j,k=1,2$;
  \item \label{assumption.BM14.symmetric_self-excitation}(symmetric self-excitation)
  $\hawkesKernel_{2k-1,2j-1}=\hawkesKernel_{2k,2j}$, for $j,k=1,2$.
 \end{enumerate}
\end{assumption}
Assumption \ref{assumption.BM14.symmetric_baseRates} says that the base rate of arrival of sell market orders is equal to that of buy market orders,
 and that the base rate at which the mid-price increases is the same as the one at which it decreases.
 In fact,
 Assumption \ref{assumption.BM14.null_price-jumps_baseRates} adds that the base rates of mid-price jumps are null.
 This is interpreted by saying that sources of exogenous information about the fundamental price of the asset exchanged are brought to the order book by market orders,
 which then may or may not trigger changes in the mid-price.
 These mid-price changes can be triggered 
either by consuming the available liquidity at some price levels (instantaneous price adjustments) 
or by causing market makers to react and move limit orders from one level to another (delayed price adjustments).
 The effects of these triggers are modelled in the Hawkes kernels $\hawkesKernel_{k,j+2}$ for $j,
k=1,2$.
% In Section \ref{sec.BM14_walking_the_book},
% we will see that \cite{BM14haw} reports that calibration on real world data showed that in fact delayed price adjustments have no explanatory power on mid-price jumps,
% and $\hawkesKernel_{1,3}$ and $\hawkesKernel_{2,4}$ will be turned into Dirac deltas to describe this.
   

Assumptions \ref{assumption.BM14.symmetric_cross-excitation} and \ref{assumption.BM14.symmetric_self-excitation} account for the symmetries between bid/ask sides of the trades and up/down jumps of the mid-price.
They result in a bloc-decomposition of the $4\times4$-matrix $\hawkesKernel$ into four $2\times2$-symmetric matrices of the form
\begin{equation*}
 \left(
 \begin{tabular}{cc}
  1 & 0 \\ 0 & 1
 \end{tabular}
 \right)s_h(t)
 +
 \left(
 \begin{tabular}{cc}
  0 & 1 \\ 1 & 0
 \end{tabular}
\right) c_h(t)
\end{equation*}
for some kernel functions $s_h(t)$ and $c_h(t)$, with $h=1,\dots,4$,
which respectively represent self-excitation and cross-excitation.
These blocs are labelled clock-wise starting from the top-left bloc.
In Section 
\ref{sec.BM14_walking_the_book}), we focus on the bloc with label $h=2$ (top-right bloc),
i.e.
on the sub-matrix $\lbrace \hawkesKernel_{\eone,e}: \, \eone =1,2; \, \, e=3,4 \rbrace$.

\subsection{Market orders walking the book}\label{sec.BM14_walking_the_book}
Assume that a trader places a buy market order (respectively,
 sell market order) of a size larger than the available liquidity on the first ask level (on the first bid level).% \footnote{In the notation of Proposition \ref{prop.lob_update},
%such orders are identified by the condition $N>1$.} 
When such an order is executed,
the limit orders sitting on the first ask (bid) level are depleted,
and as a result the mid-price increases (decreases).
When this happens,
it is said that the market order \emph{walks the book}.
We will also refer to such market orders as \emph{aggressive} market orders.


A buy (sell) market order coming into the exchange and walking the book at time $t$
would be represented in the Bacry\&Muzy model by the equation
 $\delta\countingProc[2](t) = \delta\countingProc[4](t) = 1$ 
(respectively, $\delta\countingProc[1](t) = \delta\countingProc[3](t) = 1$).
However, the components of a multidimensional Hawkes process jump simultaneously with probability zero.
In other words, 
if $\lbrace (\arrivalTimes[e]_j)_j: \, e=1,.\dots,\numEventTypes\rbrace$ are the arrival times associated with a $\numEventTypes$-dimensional Hawkes process, 
it holds 
$\Prob(\arrivalTimes[e]_j = \arrivalTimes[\eone]_{j\derivative}, \, \text{for some } j,j\derivative\geq 1, \text{ and } e\ne\eone) = 0$.

%A way around this discrepancy had therefore to be designed; Bacry and Muzy call it ``impulsive impact kernel''. 
Since the direction of the causality is unambiguous (a market order originates first and as a result of its execution the mid--price jumps), 
\cite{BM14haw} propose to allow the diagonal entries in the top-right bloc of the Hawkes kernel to posses an atomic component.
This means that,  with the notation introduced in the previous paragraph, they assume 
\begin{equation*}
 s_2(t) = \diracDelta_t + \tilde{s}_2(t),
\end{equation*}
where $\diracDelta_t$ is the Dirac delta concentrated at $t=0$, and $\tilde{s}_2 (t)$ is the non-atomic component of $s_2(t)$, i.e.
a regular non-negative Lebesgue-integrable function defined on the non-negative half line.
$\diracDelta_t$ accounts for instantaneous price adjustments when trades happen;
$\tilde{s}_2 (t)$ accounts for delayed price adjustments after trades happened.
%Notice that the atomic component in the Hawkes kernel raises interesting mathematical questions about existence of an associated Hawkes process, which the authors defer to future works.
From a numerical point of view, 
the atomic component $\diracDelta_t$ is encoded as a 
non-negative $\Lone$ function supported in some small right-neighbourhood of the origin 
and with a certain positive $\Lone$-norm.


Although a priori $\tilde{s}_2$ is not expected to be null,
the calibration on real data performed in \cite{BM14haw} finds that this is in fact the  case.
Less surprisingly, $c_2 = c_2 (t)$ is also found to be identically null 
(buy market orders have no influence on price decrease, 
and sell market orders have no influence on price increase).
Consequently, the top-right bloc in the decomposition of $\hawkesKernel$ is a multiple of a $2\times2$-identity matrix,
where the multiplying factor $s_2$ is equal to a Dirac delta concentrated in $t=0$.
This form of the top-right bloc defines the ``impulsive impact kernel''
-- see \cite[Section 2.1.3]{BM14haw}.


An impulsive impact kernel is therefore a way to model the fact that the influence of market orders on the changes in the mid-price is binary:
either they instantaneously trigger a jump, or they have no influence on the mid-price.
 In conjunction with Assumption \ref{assumption.BM14.null_price-jumps_baseRates}, this means that in Bacry\&Muzy model, exogenous information -- if any -- is carried to the order book by market orders, whose effect does not accrue over time.
Instead, it is the flow of limit orders that is responsible for those price jumps that are not a result of market orders walking the book.

%Non-market-orders-induced changes in the mid-price result either from new limit orders posted inside the spread, or from the cancellation of existing orders sitting on the first levels of either sides. The first alternative reduces the spread, the second widens it. Collectively, we refer to these modifications in the order book configuration as \emph{limit orders' re-adjustments}.   Bacry\&Muzy model does not keep track of limit orders, but captures their effect on the mid-price via the bottom-right bloc of the Hawkes kernels: $s_3=s_3(t)$ (respectively, $c_3=c_3(t)$)  models the effect that a price jump in one direction has on the likelihood of subsequent jumps in the same (opposite) direction resulting from limit orders' re-adjustments.

In Section \ref{sec.sdhawkes_model} we will present an alternative description of the order book dynamics which
 will not necessitate atomic components in the Hawkes kernel.
Crucially, this will hinge on the introduction of a state-variable $\stateVariable$ paired with the  counting process $\multiCountingProc$.


\subsection{Price impact profiles in Bacry\&Muzy model}\label{sec.BM14_price_impact_profiles}
In \citealp[Section 4]{BM14haw},
the authors study how a labelled agent's market orders can affect the evolution of the order book dynamics.
This addresses the impact of a trader's own activity on the asset's price that they are trading.
In this paragraph we describe Bacry\&Muzy approach in the case of a liquidation,
i.e.
the sale of some (usually large) amount of shares in a trading venue that operates via a limit order book.\footnote{In fact,
\cite{BM14haw} give a more general description in which the labelled agent can intervene in the market either by sell market orders,
buy market orders or both.}

Let the instant at which the liquidator becomes active in the market be the origin of time.
Let $A(t)$ be the number of sell market orders sent by the liquidator before time  $t$.
The map $t\mapsto A(t)$ is called execution schedule, 
and describes how the liquidator is distributing the overall sale, or  \emph{metaorder}, over time.
In practice, the metaorder comprises several smaller \emph{child orders}, 
and $A$ is thought of as a description of the rate of their execution during the time window $[0,\timeHorizon)$.
Notice, however, that the sizes of the child orders are left out from the model. 

From the point of view of the trading mechanism,
$A(t)$ is similar to the first component $\countingProc[1](t)$ of the four-dimensional Hawkes process $\multiCountingProc(t)$ around which the order book dynamics are modelled:
while $\countingProc[1](t)$ represents the aggregate anonymous quantity of sell market orders that all the market participants other than the liquidator have sent to the order book by time $t$,
$A(t)$ represents the identifiable orders sent by the liquidator.
 However,
the mathematical representation of $A(t)$ is different from that of  $\countingProc[1](t)$.
Indeed,
$A(t)$ is assumed to be a non-negative non-decreasing right-continuous deterministic function,
such that the associated measure $dA(t)$ is supported in the half-open interval $[0,\timeHorizon)$,
for some $\timeHorizon>0$ representing the time horizon of the liquidation.

The presence of the liquidator affects the dynamics of the order book by contributing to the intensities of $\multiCountingProc$.
For $e=1,\dots,4$ and $t>0$ it is set 
\begin{equation}\label{eq.BM14_intensity_with_liquidator}
 \intensity[e](t) = 
 \baseRate_e
 +\sum_{\eone=1}^{4}\int_{[0,t)} \hawkesKernel\subscriptee (t-s)d\countingProc[\eone](s) 
 + \int_{[0,t)} \theta_e(s)dA(s),
\end{equation}
where $\theta_1 = \theta_1(t)$ 
(respectively, $\theta_2=\theta_2(t)$)
represents the impact of the liquidator's market orders on the arrival of other participants' sell (buy) market orders,
and $\theta_3 = \theta_3(t)$ 
(respectively, $\theta_4 = \theta_4(t)$) 
represents the impact of the liquidator's market orders on downward (upward) jumps of the mid-price.

Notice that, from the point of view of the study of price impact, $\theta_3(t)$ and $\theta_4(t)$ are crucial aspects of the model.
For consistency, liquidator's market orders are assumed to impact the  price in the same way that other participants' orders do. 
Therefore,
it is set $\theta_3(t) = \hawkesKernel_{1,3}(t) = s_2(t)$ and $\theta_4(t)=\hawkesKernel_{1,4}(t)=c_2(t)=0$.
Practically, this translates into the fact that 
the measure of the liquidator's price impact is mapped back to the estimated overall impact of other participants' market orders, 
and the liquidator's impact profile will result from the combination of the execution schedule $A(t)$ with these estimates.

%More precisely, the price impact is assessed as follows.
%Because of the assumed symmetries (Assumption \ref{assumption.BM14}), in the absence of the liquidator (i.e.
%when $A\equiv 0$), the expected price movement $\Expectation [\countingProc[4](t) - \countingProc[3](t)]$ is null for all $t$.
%Instead, when $A(t)$ is non-constant,  the liquidator's intervention tends to depress this expected price.
%It is therefore the expected curve $t\mapsto \Expectation[\countingProc[4](t)-\countingProc[3](t)]$ that is defined as the price impact profile.
%A closed-form formula for this expectation is derived in \cite[Proposition 5.1 and Corollary 5.2]{BM14haw}, where indeed the main ingredients are the execution schedule $A(t)$ and the functions $s_h(t)$, $c_h(t)$, for $h=1,\dots,4$.
%The closed-form formula has also the merit to reconcile this rather theoretical measurement with more empirical ones such as \cite{BN13mar} and  \cite{MVMGFVLM09mar}.
Indeed,
recall from  Section \ref{sec.BM14_walking_the_book} that market orders have binary effects on price movements:
either they deplete the available liquidity sitting at the best bid/ask prices (they walk the book), or they have no influence on the mid-price (when the liquidity that they demand is fully serviced by limit orders sitting on level 1 of either sides).
Assuming that the liquidator's market orders impact the price jumps in the same way as other market orders do would therefore imply that the liquidator chooses to walk the book at an average rate equal to the overall proportion of aggressive market orders.
 

In Section \ref{sec.price_impact_profiles},
we propose an assessment of price impct profiles that differs from Bacry and Muzy's in three ways.
Firstly,
we give a measurement of the impact profile that is scenario-dependent,
i.e.
we refrain from measuring the \emph{average} impact,
yet factoring out the ``noise'' associated with the random evolution of the order book dynamics.
Secondly,
we account for stochastic execution schedule $A(t)$,
bringing the mathematical description of them closer to the one of $\countingProc[1](t)$.
Thirdly,
we do not assume that the liquidator's market orders impact the price jumps in the same way as other market orders do.



==> sections/bm14_model.tex <==
\subsection{Model description}
Two aspects of the time evolution of the order-driven market are modelled:
trades and changes in the mid-price.
% As explained in Section \ref{sec.order-driven_markets}, 
Trades can in fact be identified with submissions of market orders, and we will do this here.

Four streams of arrival times are considered:
the stream $(\arrivalTimes[1]_j)_j$ of times when limit orders are executed on the bid side
(equivalently identified with the arrival times of sell market orders);
the stream  $(\arrivalTimes[2]_j)_j$ of times when limit orders are executed on the ask side
(equivalently identified with arrival times of buy market orders);
the stream  $(\arrivalTimes[3]_j)_j$ of times when the mid-price decreases;
the stream  $(\arrivalTimes[4]_j)_j$ of times when the mid-price increases. 
Correspondingly, these sequences of random times give rise to a four-dimensional counting process $\multiCountingProc=(\countingProc[1],\dots, \countingProc[4])$ with the following interpretation of its components:
\begin{itemize}
 \item $\countingProc[1](t)$ denotes the number of seller-initiated trades that happened before or at time $t$
(identified with the number of market orders arrived on the bid side of the order book by time $t$);
 \item $\countingProc[2](t)$ denotes the number of buyer-initiated trades that happened before or at time $t$
(identified with the number of market orders arrived on the ask side of the order book by time $t$);
 \item $\countingProc[3](t)$ denotes the number of downward jumps of the mid-price  that happened before or at time $t$;
 \item $\countingProc[4](t)$ denotes the number of upward jumps of the mid-price  that happened before or at time $t$.
\end{itemize}

Notice that $\countingProc[4]-\countingProc[3]$ is a proxy for the mid-price.
Indeed,
given the tick size $\tickSizeOfLOB$ of the limit order book and the initial position $\midprice_0$ of the mid-price,
 the paths $t\mapsto \midprice_0 +(\countingProc[4](t)-\countingProc[3](t))\tickSizeOfLOB$ and $t\mapsto \midprice_t$ will have discrepancies only when $\vert\delta\midprice(t)\vert \geq 2\tickSizeOfLOB$,
and this rarely happens (in particular for limit order books with large tick size).

The counting process $\multiCountingProc$ is assumed to be an ordinary Hawkes process,
hence it admits a continuous compensator with an intensity $\intensity[]=(\intensity[1],\dots,\intensity[4])$ of the type in equation \eqref{eq.intensity_ordHawkes}.
 We let $\baseRate$ be the $4$-dimensional vector of base rates, and we let $\hawkesKernel$ be the $4\times4$-dimensional matrix of Hawkes kernels.
 In the model of \cite{BM14haw}, the following assumptions are in place on the so-introduced four-dimensional Hawkes process:
\begin{assumption}\label{assumption.BM14}
 \begin{enumerate}[label={\emph{\roman{*}}.} , ref={\ref{assumption.BM14}.\emph{\roman{*}}}]
  \item\label{assumption.BM14.symmetric_baseRates} (symmetric base rates)
  $\baseRate_{2k-1}=\baseRate_{2k}$,  for $k=1,2$;
  \item\label{assumption.BM14.null_price-jumps_baseRates} (fully endogenous price jumps) $\baseRate_3 = \baseRate_4=0$;
  \item \label{assumption.BM14.symmetric_cross-excitation}(symmetric cross-excitation)
  $\hawkesKernel_{2k-1,2j}=\hawkesKernel_{2j,2k-1}$, for $j,k=1,2$;
  \item \label{assumption.BM14.symmetric_self-excitation}(symmetric self-excitation)
  $\hawkesKernel_{2k-1,2j-1}=\hawkesKernel_{2k,2j}$, for $j,k=1,2$.
 \end{enumerate}
\end{assumption}
Assumption \ref{assumption.BM14.symmetric_baseRates} says that the base rate of arrival of sell market orders is equal to that of buy market orders,
 and that the base rate at which the mid-price increases is the same as the one at which it decreases.
 In fact,
 Assumption \ref{assumption.BM14.null_price-jumps_baseRates} adds that the base rates of mid-price jumps are null.
 This is interpreted by saying that sources of exogenous information about the fundamental price of the asset exchanged are brought to the order book by market orders,
 which then may or may not trigger changes in the mid-price.
 These mid-price changes can be triggered 
either by consuming the available liquidity at some price levels (instantaneous price adjustments) 
or by causing market makers to react and move limit orders from one level to another (delayed price adjustments).
 The effects of these triggers are modelled in the Hawkes kernels $\hawkesKernel_{k,j+2}$ for $j,
k=1,2$.
% In Section \ref{sec.BM14_walking_the_book},
% we will see that \cite{BM14haw} reports that calibration on real world data showed that in fact delayed price adjustments have no explanatory power on mid-price jumps,
% and $\hawkesKernel_{1,3}$ and $\hawkesKernel_{2,4}$ will be turned into Dirac deltas to describe this.
   

Assumptions \ref{assumption.BM14.symmetric_cross-excitation} and \ref{assumption.BM14.symmetric_self-excitation} account for the symmetries between bid/ask sides of the trades and up/down jumps of the mid-price.
They result in a bloc-decomposition of the $4\times4$-matrix $\hawkesKernel$ into four $2\times2$-symmetric matrices of the form
\begin{equation*}
 \left(
 \begin{tabular}{cc}
  1 & 0 \\ 0 & 1
 \end{tabular}
 \right)s_h(t)
 +
 \left(
 \begin{tabular}{cc}
  0 & 1 \\ 1 & 0
 \end{tabular}
\right) c_h(t)
\end{equation*}
for some kernel functions $s_h(t)$ and $c_h(t)$, with $h=1,\dots,4$,
which respectively represent self-excitation and cross-excitation.
These blocs are labelled clock-wise starting from the top-left bloc.
In Section 
\ref{sec.BM14_walking_the_book}), we focus on the bloc with label $h=2$ (top-right bloc),
i.e.
on the sub-matrix $\lbrace \hawkesKernel_{\eone,e}: \, \eone =1,2; \, \, e=3,4 \rbrace$.

\subsection{Market orders walking the book}\label{sec.BM14_walking_the_book}
Assume that a trader places a buy market order (resp.,
 sell market order) of a size larger than the available liquidity on the first ask level (on the first bid level).% \footnote{In the notation of Proposition \ref{prop.lob_update},
%such orders are identified by the condition $N>1$.} 
When such an order is executed,
the limit orders sitting on the first ask (bid) level are depleted,
and as a result the mid-price increases (decreases).
When this happens,
it is said that the market order \emph{walks the book}.
We will also refer to such market orders as \emph{aggressive} market orders.


A buy (sell) market order coming into the exchange and walking the book at time $t$
would be represented in the Bacry\&Muzy model by the equation
 $\delta\countingProc[2](t) = \delta\countingProc[4](t) = 1$ 
(resp., $\delta\countingProc[1](t) = \delta\countingProc[3](t) = 1$).
However, the components of a multidimensional Hawkes process jump simultaneously with probability zero.
In other words, 
if $\lbrace (\arrivalTimes[e]_j)_j: \, e=1,.\dots,\numEventTypes\rbrace$ are the arrival times associated with a $\numEventTypes$-dimensional Hawkes process, 
it holds 
$\Prob(\arrivalTimes[e]_j = \arrivalTimes[\eone]_{j\derivative}, \, \text{for some } j,j\derivative\geq 1, \text{ and } e\ne\eone) = 0$.

%A way around this discrepancy had therefore to be designed; Bacry and Muzy call it ``impulsive impact kernel''. 
Since the direction of the causality is unambiguous (a market order originates first and as a result of its execution the mid--price jumps), 
\cite{BM14haw} propose to allow the diagonal entries in the top-right bloc of the Hawkes kernel to posses an atomic component.
This means that,  with the notation introduced in the previous paragraph, they assume 
\begin{equation*}
 s_2(t) = \diracDelta_t + \tilde{s}_2(t),
\end{equation*}
where $\diracDelta_t$ is the Dirac delta concentrated at $t=0$, and $\tilde{s}_2 (t)$ is the non-atomic component of $s_2(t)$, i.e.
a regular non-negative Lebesgue-integrable function defined on the non-negative half line.
$\diracDelta_t$ accounts for instantaneous price adjustments when trades happen;
$\tilde{s}_2 (t)$ accounts for delayed price adjustments after trades happened.
%Notice that the atomic component in the Hawkes kernel raises interesting mathematical questions about existence of an associated Hawkes process, which the authors defer to future works.
From a numerical point of view, 
the atomic component $\diracDelta_t$ is encoded as a 
non-negative $\Lone$ function supported in some small right-neighbourhood of the origin 
and with a certain positive $\Lone$-norm.


Although a priori $\tilde{s}_2$ is not expected to be null,
the calibration on real data performed in \cite{BM14haw} finds that this is in fact the  case.
Less surprisingly, $c_2 = c_2 (t)$ is also found to be identically null 
(buy market orders have no influence on price decrease, 
and sell market orders have no influence on price increase).
Consequently, the top-right bloc in the decomposition of $\hawkesKernel$ is a multiple of a $2\times2$-identity matrix,
where the multiplying factor $s_2$ is equal to a Dirac delta concentrated in $t=0$.
This form of the top-right bloc defines the ``impulsive impact kernel''
-- see \cite[Section 2.1.3]{BM14haw}.


An impulsive impact kernel is therefore a way to model the fact that the influence of market orders on the changes in the mid-price is binary:
either they instantaneously trigger a jump, or they have no influence on the mid-price.
 In conjunction with Assumption \ref{assumption.BM14.null_price-jumps_baseRates}, this means that in Bacry\&Muzy model, exogenous information -- if any -- is carried to the order book by market orders, whose effect does not accrue over time.
Instead, it is the flow of limit orders that is responsible for those price jumps that are not a result of market orders walking the book.

%Non-market-orders-induced changes in the mid-price result either from new limit orders posted inside the spread, or from the cancellation of existing orders sitting on the first levels of either sides. The first alternative reduces the spread, the second widens it. Collectively, we refer to these modifications in the order book configuration as \emph{limit orders' re-adjustments}.   Bacry\&Muzy model does not keep track of limit orders, but captures their effect on the mid-price via the bottom-right bloc of the Hawkes kernels: $s_3=s_3(t)$ (respectively, $c_3=c_3(t)$)  models the effect that a price jump in one direction has on the likelihood of subsequent jumps in the same (opposite) direction resulting from limit orders' re-adjustments.

In Section \ref{sec.sdhawkes_model} we will present an alternative description of the order book dynamics which
 will not necessitate atomic components in the Hawkes kernel.
Crucially, this will hinge on the introduction of a state-variable $\stateVariable$ paired with the  counting process $\multiCountingProc$.


\subsection{Price impact profiles in Bacry\&Muzy model}\label{sec.BM14_price_impact_profiles}
In \citealp[Section 4]{BM14haw},
the authors study how a labelled agent's market orders can affect the evolution of the order book dynamics.
This addresses the impact of a trader's own activity on the asset's price that they are trading.
In this paragraph we describe Bacry\&Muzy approach in the case of a liquidation,
i.e.
the sale of some (usually large) amount of shares in a trading venue that operates via a limit order book.\footnote{In fact,
\cite{BM14haw} give a more general description in which the labelled agent can intervene in the market either by sell market orders,
buy market orders or both.}

Let the instant at which the liquidator becomes active in the market be the origin of time.
Let $A(t)$ be the number of sell market orders sent by the liquidator before time  $t$.
The map $t\mapsto A(t)$ is called execution schedule, 
and describes how the liquidator is distributing the overall sale, or  \emph{metaorder}, over time.
In practice, the metaorder comprises several smaller \emph{child orders}, 
and $A$ is thought of as a description of the rate of their execution during the time window $[0,\timeHorizon)$.
Notice, however, that the sizes of the child orders are left out from the model. 

From the point of view of the trading mechanism,
$A(t)$ is similar to the first component $\countingProc[1](t)$ of the four-dimensional Hawkes process $\multiCountingProc(t)$ around which the order book dynamics are modelled:
while $\countingProc[1](t)$ represents the aggregate anonymous quantity of sell market orders that all the market participants other than the liquidator have sent to the order book by time $t$,
$A(t)$ represents the identifiable orders sent by the liquidator.
 However,
the mathematical representation of $A(t)$ is different from that of  $\countingProc[1](t)$.
Indeed,
$A(t)$ is assumed to be a non-negative non-decreasing right-continuous deterministic function,
such that the associated measure $dA(t)$ is supported in the half-open interval $[0,\timeHorizon)$,
for some $\timeHorizon>0$ representing the time horizon of the liquidation.

The presence of the liquidator affects the dynamics of the order book by contributing to the intensities of $\multiCountingProc$.
For $e=1,\dots,4$ and $t>0$ it is set 
\begin{equation}\label{eq.BM14_intensity_with_liquidator}
 \intensity[e](t) = 
 \baseRate_e
 +\sum_{\eone=1}^{4}\int_{[0,t)} \hawkesKernel\subscriptee (t-s)d\countingProc[\eone](s) 
 + \int_{[0,t)} \theta_e(s)dA(s),
\end{equation}
where $\theta_1 = \theta_1(t)$ 
(resp., $\theta_2=\theta_2(t)$)
represents the impact of the liquidator's market orders on the arrival of other participants' sell (buy) market orders,
and $\theta_3 = \theta_3(t)$ 
(resp., $\theta_4 = \theta_4(t)$) 
represents the impact of the liquidator's market orders on downward (upward) jumps of the mid-price.

Notice that, from the point of view of the study of price impact, $\theta_3(t)$ and $\theta_4(t)$ are crucial aspects of the model.
For consistency, liquidator's market orders are assumed to impact the  price in the same way that other participants' orders do. 
Therefore,
it is set $\theta_3(t) = \hawkesKernel_{1,3}(t) = s_2(t)$ and $\theta_4(t)=\hawkesKernel_{1,4}(t)=c_2(t)=0$.
Practically, this translates into the fact that 
the measure of the liquidator's price impact is mapped back to the estimated overall impact of other participants' market orders, 
and the liquidator's impact profile will result from the combination of the execution schedule $A(t)$ with these estimates.

%More precisely, the price impact is assessed as follows.
%Because of the assumed symmetries (Assumption \ref{assumption.BM14}), in the absence of the liquidator (i.e.
%when $A\equiv 0$), the expected price movement $\Expectation [\countingProc[4](t) - \countingProc[3](t)]$ is null for all $t$.
%Instead, when $A(t)$ is non-constant,  the liquidator's intervention tends to depress this expected price.
%It is therefore the expected curve $t\mapsto \Expectation[\countingProc[4](t)-\countingProc[3](t)]$ that is defined as the price impact profile.
%A closed-form formula for this expectation is derived in \cite[Proposition 5.1 and Corollary 5.2]{BM14haw}, where indeed the main ingredients are the execution schedule $A(t)$ and the functions $s_h(t)$, $c_h(t)$, for $h=1,\dots,4$.
%The closed-form formula has also the merit to reconcile this rather theoretical measurement with more empirical ones such as \cite{BN13mar} and  \cite{MVMGFVLM09mar}.
Indeed,
recall from  Section \ref{sec.BM14_walking_the_book} that market orders have binary effects on price movements:
either they deplete the available liquidity sitting at the best bid/ask prices (they walk the book), or they have no influence on the mid-price (when the liquidity that they demand is fully serviced by limit orders sitting on level 1 of either sides).
Assuming that the liquidator's market orders impact the price jumps in the same way as other market orders do would therefore imply that the liquidator chooses to walk the book at an average rate equal to the overall proportion of aggressive market orders.
 

In Section \ref{sec.price_impact_profiles},
we propose an assessment of price impact profiles that differs from Bacry and Muzy's in three ways.
Firstly,
we give a measurement of the impact profile that is scenario-dependent,
i.e.
we refrain from measuring the \emph{average} impact,
yet factoring out the ``noise'' associated with the random evolution of the order book dynamics.
Secondly,
we account for stochastic execution schedule $A(t)$,
bringing the mathematical description of them closer to the one of $\countingProc[1](t)$.
Thirdly,
we do not assume that the liquidator's market orders impact the price jumps in the same way as other market orders do.


